Quantum Algorithms for solving Hard Constrained Optimisation Problems

The thesis deals with Quantum Algorithms for solving Hard Constrained Optimization Problems. It shows how quantum computers can solve difficult everyday problems such as finding the best schedule for social workers or the path of a robot picking and batching in a warehouse. The path to the solution has led to the definition of a new artificial intelligence paradigm with quantum computing, quantum Case-Based Reasoning (qCBR) and to a proof of concept to integrate the capacity of quantum computing within mobile robotics using a Raspberry Pi 4 as a processor (qRobot), capable of operating with leading technology players such as IBMQ, Amazon Braket (D-Wave) and Pennylane. To improve the execution time of variational algorithms in this NISQ era and the next, we have proposed EVA: a quantum Exponential Value Approximation algorithm that speeds up the VQE, and that is, to date, the flagship of the quantum computation. To improve the execution time of variational algorithms in this NISQ era and the next, we have proposed EVA: a quantum Exponential Value Approximation algorithm that speeds up the VQE, and that is, to date, the flagship of the quantum computation.

==> Annex.tex <==
\newpage

\chapter{Annex} \label{sec:Appendix}
In this section we will add the useful Appendix for the best understanding of this PhD work.
\section{Cost Function}\label{sec:Poli_NP}
To dive deeply into Cost function analyzing, this ref. \cite{Nikolova2002} is more adequate.

\section{Installation of ARM64 on Raspberry Pi 4}\label{sec:InstallationARM64}
The description step by step into how installing and running Pennylane, AWS-Braket, D-Wave-Ocean, Qiskit, on a Raspberry Pi 4 under the ARM64\cite{jiang2020power} operating system turn it into a quantum computing simulator and use it to access real quantum computers from IBMQ\cite{Qis21,mckay2018qiskit}, AWS-Braket\cite{AWS_Braket}, D-Wave\cite{dwave_computer}, and Regetti\cite{sete2016functional}. These frameworks and packages are required for the proof of concept that we propose \cite{qRobotP}.
\begin{figure}[!ht]
\centering
\includegraphics[width=0.75\textwidth]{media/qRobot_Platform.png}
\caption{We have installed the following frameworks successfully (Qiskit, Pennylane, AWS-Braket) on our Raspberry Pi 4 under the ARM64 operating system. More information about the qRobot platform can be found at Ref.~\cite{qRobotP}}
\label{fig:qRobot_platform}
\end{figure}







\section{Summary}
In this chapter, we have seen the results, the discussions, the conclusions and the future lines of this thesis. However, if the reader would like more details, we would recommend them to the chapter of each of the projects developed to answer the question of this thesis. In this case, could we use quantum computation to solve combinatorial optimization problems with hard constraints?

==> myContributions.tex <==
%\section* {My contributions to this PhD thesis}
\subsection*{Pedagogical contribution} \label{sec:myContr_pedago}
\begin{itemize}
    \item Some guidelines and steps to solve combinatorial optimization problems in quantum.
    \item A documentation of the state of the art and compilation and access to the main tutorials of quantum frameworks
    \item a GitHub with the codes and experimentation environments
    \item Complete formulation of a real combinatorial optimization problem (SWP) with restrictions and mapping it in quantum.
    \item Step-by-step development of how to bring a classical to a quantum optimization problem (SWP)
    \item Design, implementation and results of the SWP Top-down resolution and quantum Case-Based Reasoning
    \item Design, implementation and comparisons of a variational quantum classifier.
    \item Design, implementation of a universal quantum platform using Raspberry PI.
    \item Design, implementation and comparisons of a picking and batching problem.
    \item co-accompany a group of collaborators in quantum computing for DS4DS
    \item Co-direction of a TFG in quantum computing
\end{itemize}

\subsection*{International contribution and talent pool}\label{sec:myContr_talent}
\begin{itemize}
    \item 8 articles
    \item Finalist in the QHack organised by Xanadu (2021)
    \item More than 20 seminars, $R\And D$ activities
    \item qRobot has Been Selected as an Issue Cover (mdpi journal)
    \item 3 congresses
    \item Worldwide connection of the DS4DS group to the quantum scientific community, IBMQ, Quantum Hispania, ORTools, AWS-Braket, Pennylane...
    \item  Contact of guru, influencer and leaders in quantum computing
\end{itemize}
\subsection*{Contribution to business vision}\label{sec:myContr_Busi}
\begin{itemize}
    \item The group could particularise one of my formulations as a Fintech product and base it on the cloud. Developing a subscription/use business model; Pay peruse.
\end{itemize}

\subsection*{What I have learned (Hard Skills)}\label{sec:myContr_what_I_learned}
\begin{itemize}
\item Quantum mechanics applied to quantum computing
\item Qiskit, Qibo, Pennylane, D-Wave, ... programming environments
\item Mathematical formulations of optimization problems
\item Mapping of classical combinatorial optimization problems in quantum
\item Design and implement classical and quantum classifiers
\item Understand quantum Machine Learning.
\item Write articles
\item Scientific rigour
\item Quantum computing.
\item The era in which quantum computing is found.
\end{itemize}

\subsection*{What I have consolidated (Soft Skills)} \label{sec:myContr_Soft_skills}
\begin{itemize}
\item Self-motivation
\item Overcome the obstacles
\item Find my life
\end{itemize}
